DeepTrack: Lightweight Deep Learning for Vehicle Path Prediction in Highways

Vehicle trajectory prediction is essential for enabling safety-critical intelligent transportation systems (ITS) applications used in management and operations. While there have been some promising advances in the field, there is a need for modern deep learning algorithms that allow real-time trajectory prediction on embedded IoT devices. This article presents DeepTrack, a novel deep learning algorithm customized for real-time vehicle trajectory prediction and monitoring applications in arterial management, freeway management, traffic incident management, and work zone management for high-speed incoming traffic. In contrast to previous methods, the vehicle dynamics are encoded using Temporal Convolutional Networks (TCNs) to provide more robust time prediction with less computation. DeepTrack also uses depthwise convolution, which reduces the complexity of models compared to existing approaches in terms of model size and operations. Overall, our experimental results demonstrate that DeepTrack achieves comparable accuracy to state-of-the-art trajectory prediction models but with smaller model sizes and lower computational complexity, making it more suitable for real-world deployment.

==> Tables/accuracy.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\iffalse
\begin{table}[htbp]
  \centering
  \caption{Performance comparison based on NGSIM dataset. RMSE is calculated in meters.}
    \begin{tabular}{lcccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Model}}} & \multicolumn{5}{c}{\textbf{RMSE (m)}} & \multirow{2}[4]{*}{\textbf{ADE}} \\
\cmidrule{2-6}          & \textbf{1 sec} & \textbf{2 sec} & \textbf{3 sec} & \textbf{4 sec} & \textbf{5 sec} &  \\
    \midrule
    CS-LSTM \cite{deo2018convolutional} & 0.61  & 1.27  & 2.09  & 3.1   & 4.37  & 2.29 \\
    CS-LSTM (M) \cite{deo2018convolutional} & 0.62  & 1.29  & 2.13  & 3.2   & 4.52  & 2.35 \\
    CF-LSTM \cite{xie2021congestion} & 0.51  & 1.13  & 1.88  & 2.81  & 3.98  & 2.06 \\
    SAAMP \cite{mercat2020multi} & 0.55  & 1.1   & 1.78  & 2.73  & 3.82  & 2.00 \\
    DeepTrack & 0.43  & 1.12  & 1.91  & 2.87  & 4.07  & 2.08 \\
    \bottomrule
    \end{tabular}%
  \label{tab:rmse}%
\end{table}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Performance comparison based on NGSIM dataset. RMSE is calculated in meters.}
    \begin{tabular}{lrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Models}}} & \multicolumn{5}{c}{\textbf{RMSE (m)}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{ADE}}} \\
\cmidrule{2-6}          & \multicolumn{1}{c}{\textbf{1 sec}} & \multicolumn{1}{c}{\textbf{2 sec}} & \multicolumn{1}{c}{\textbf{3 sec}} & \multicolumn{1}{c}{\textbf{4 sec}} & \multicolumn{1}{c}{\textbf{5 secs}} &  \\
    \midrule
    CS-LSTM \cite{deo2018convolutional} & 0.61  & 1.27  & 2.09  & 3.1   & 4.37  & 2.29 \\
    CF-LSTM \cite{xie2021congestion} & 0.55  & 1.10   & 1.78  & 2.73  & 3.82  & 2.06 \\
    SAAMP \cite{mercat2020multi} & 0.51  & 1.13  & 1.88  & 2.81  & 3.98  & 2.00 \\
    STA-LSTM \cite{lin2020attention}& 0.37  & 0.98  & 1.71  & 2.63  & 3.78  & 1.89 \\
    DeepTrack & 0.43  & 1.12  & 1.95  & 2.97  & 4.23  & 2.08 \\
    DeepTrack-ATT & 0.43  & 1.09  & 1.87   & 2.80   & 3.94  & 2.03 \\
    \bottomrule
    \end{tabular}%
  \label{tab:rmse}%
\end{table}%
\fi

\iffalse
% Table generated by Excel2LaTeX from sheet 'Sheet5'
\begin{table}[htbp]
  \centering
  \caption{Performance comparison based on NGSIM dataset. RMSE is calculated in meters.}
    \begin{tabular}{ccccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Model}}} & \multicolumn{5}{c}{\textbf{RMSE (m)}} & \multirow{2}[4]{*}{\textbf{ADE}} \\
\cmidrule{2-6}          & \textbf{1 sec} & \textbf{2 sec} & \textbf{3 sec} & \textbf{4 sec} & \textbf{5 sec} &  \\
    \midrule
    CS-LSTM \cite{deo2018convolutional} & 0.61  & 1.27  & 2.09  & 3.10   & 4.37  & 2.29 \\
    CF-LSTM \cite{xie2021congestion} & 0.51  & 1.13  & 1.88  & 2.81  & 3.98  & 2.06 \\
    SAAMP \cite{mercat2020multi} & 0.55  & 1.10   & 1.78  & 2.73  & 3.82  & 2.00 \\
    STA-LSTM \cite{lin2020attention} & 0.37  & 0.98  & 1.71  & 2.63  & 3.78  & 1.89 \\
    DeepTrack-ATT & 0.46  & 1.07  & 1.84  & 2.78  & 3.93  & 2.01 \\
    \bottomrule
    \end{tabular}%
  \label{tab:rmse}%
      \vspace{-10pt}
\end{table}%
\fi

% Table generated by Excel2LaTeX from sheet 'Sheet5'
\begin{table}[htbp]
  \centering
  \caption{Performance comparison based on NGSIM dataset. RMSE is calculated in meters.}
    \begin{tabular}{cccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Model}}} & \multicolumn{5}{c}{\textbf{RMSE (m)}} \\
\cmidrule{2-6}          & \textbf{1 sec} & \textbf{2 sec} & \textbf{3 sec} & \textbf{4 sec} & \textbf{5 sec}  \\
    \midrule
    CS-LSTM \cite{deo2018convolutional} & 0.61  & 1.27  & 2.09  & 3.10   & 4.37 \\
    CF-LSTM \cite{xie2021congestion} & 0.51  & 1.13  & 1.88  & 2.81  & 3.98 \\
    SAAMP \cite{mercat2020multi} & 0.55  & 1.10   & 1.78  & 2.73  & 3.82 \\
    STA-LSTM \cite{lin2020attention} & 0.37  & 0.98  & 1.71  & 2.63  & 3.78\\
    DeepTrack-ATT & 0.46  & 1.07  & 1.84  & 2.78  & 3.93\\
    \bottomrule
    \end{tabular}%
  \label{tab:rmse}%
      \vspace{-10pt}
\end{table}%


% Table generated by Excel2LaTeX from sheet 'ReLU6'
\begin{table}[htbp]
  \centering
  \caption{FDE and ADE Performance comparison based on NGSIM dataset.}
    \begin{tabular}{ccc}
    \toprule
    \textbf{Models} & \multicolumn{1}{p{4.055em}}{\textbf{FDE (m)}} & \multicolumn{1}{p{4.055em}}{\textbf{ADE (m)}} \\
    \midrule
    CS-LSTM &  3.34  & 2.29 \\
    CF-LSTM &       & 2.06 \\
    SAAMP &       & 2 \\
    STA-LSTM &  3.16     & 1.89 \\
    DeepTrack & 3.25  & 2.01 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%



==> Tables/flops.tex <==
\begin{table}[htbp]
  \centering
  \caption{Model size and number of MACs per model}
  \begin{adjustbox}{width=0.8\linewidth}
     \begin{tabular}{p{6.39em}cc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Model}}} & \multicolumn{2}{c}{\textbf{Parameters}} \\
\cmidrule{2-3}    \multicolumn{1}{c}{} & \textbf{MACs} & \textbf{Parameters} \\
    \midrule
    \multicolumn{1}{l}{CS-LSTM \cite{deo2018convolutional}} & 3,580,392 & 191,829 \\
    \multicolumn{1}{l}{CF-LSTM \cite{xie2021congestion}} & 3,612,494 & 193,941 \\
    \multicolumn{1}{l}{STA-LSTM \cite{lin2020attention}} & 3,634,456 & 124,835 \\
    \multicolumn{1}{l}{DeepTrack-ATT} & \textbf{\red{2,804,419}} & \textbf{109,099} \\
    \bottomrule
        \vspace{-15pt}
    \end{tabular}%
    \vspace{-15pt}    
  \end{adjustbox}
  \label{tab:flops}%
\end{table}%

